Workload Balancing Among Heathcare Workers Under Uncertain Service Time Using Distributionally Robust Optimization

Healthcare systems are facing serious challenges in balancing their human resources to cope with volatile service demand, while at the same time providing necessary job satisfaction to the healthcare workers. We propose in this paper a distributionally robust optimization formulation to generate a task assignment plan that promotes the fairness in allocation, attained by reducing the difference in the total working time among workers, under uncertain service time. The proposed joint chance constraint model is conservatively approximated by a worst-case Conditional Value-at-Risk, and we devise a sequential algorithm to solve the finite-dimensional reformulations which are linear (mixed-binary) optimization problems. We also provide explicit formula in the situation where the support set of the random vectors is a hyperrectangle. The experiment with synthetic data suggests promising results for our approach.

==> Workload Balancing/comments.tex <==
% for underbar
\makeatletter
\def\munderbar#1{\underline{\sbox\tw@{$#1$}\dp\tw@\z@\box\tw@}}
\makeatother


\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{example}[theorem]{Example}
%==================================

\newcommand{\viet}[1]{\textbf{{\color{magenta}(#1)}}}

%======================================
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{equation*}\begin{aligned}}
\newcommand{\eea}{\end{aligned}\end{equation*}}
\newcommand{\ds}{\displaystyle}
\newcommand{\independent}{\protect\mathpalette{\protect\independenT}{\perp}}
\newcommand{\R}{\mathbb{R}}

\newcommand{\Max}{\max\limits_}
\newcommand{\Min}{\min\limits_}
\newcommand{\Sup}{\sup\limits_}
\newcommand{\Inf}{\inf\limits_}
\newcommand{\st}{\mathrm{s.t.}}

\newcommand{\wh}{\widehat}
\newcommand{\mc}{\mathcal}
\newcommand{\mbb}{\mathbb}
\newcommand{\inner}[2]{\big \langle #1, #2 \big \rangle }
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\cov}{\Sigma} % true covariance matrix
\newcommand{\covinv}{\Sigma^{-1}} % true precision matrix
\newcommand{\covsa}{\wh{\Sigma}} % covariance sample average

\newcommand{\PP}{\mbb P}
\newcommand{\Pnom}{\wh{\mbb P}}
\newcommand{\QQ}{\mbb Q}
\newcommand{\DD}{\mbb D}

\newcommand{\Struct}{\mc S} % structural set
\newcommand{\Ambi}{\mc P} % Ambiguity set
\newcommand{\LHSfunction}{\phi_\rho}

%\newcommand{\est}{X\opt}
%\newcommand{\estL}{\lambda\opt}
%\newcommand{\estx}{x\opt}



\newcommand{\defeq}{%
  \mathrel{\vbox{\offinterlineskip\ialign{%
    \hfil##\hfil\cr
    $\scriptscriptstyle\triangle$\cr
    %\noalign{\kern0ex}
    $=$\cr
}}}}

% Peyman's comments
\newcommand{\PSD}{\mathbb{S}_{+}} % the set of positive semi-definite matrices of dimension p
\newcommand{\PD}{\mathbb{S}_{++}} % the set of positive semi-definite matrices of dimension p
\newcommand{\Let}{\triangleq}
\newcommand{\opt}{^\star}
\newcommand{\eps}{\varepsilon}
\newcommand{\ra}{\rightarrow}
\newcommand{\M}{\mc M}
\newcommand{\BB}{\mbb B}
\newcommand{\B}{\mc B}
\newcommand{\X}{X}
\newcommand{\Y}{Y}
\newcommand{\Wass}{\mathds{W}}
\newcommand{\V}{\mathds{W}_S}
\newcommand{\Q}{\mbb{Q}}
\newcommand{\EE}{\mathds{E}}
\newcommand{\tr}{\intercal}
\newcommand{\Xset}{\mc X}

\newcommand{\half}{\frac{1}{2}}
\newcommand{\dualvar}{\gamma}

\newcommand{\auxfunc}{\omega}
\newcommand{\covsaeig}{\lambda}
\newcommand{\covsaeigvect}{v}
\newcommand{\ie}{{\em i.e.}}
\newcommand{\da}{\downarrow}
\newcommand{\J}{\mc J}
\newcommand{\Dataset}{\wh{\mc D}}

\newcommand{\p}{\mathbb P}
\newcommand{\psa}{\wh \p}
\newcommand{\N}{\mathcal N}
\newcommand{\f}{f}
\newcommand{\g}{g}
\newcommand{\radius}{\rho}
\newcommand{\Sym}{\mbb S}
\newcommand{\m}{\mu}
\newcommand{\msa}{\wh \m}



==> Workload Balancing/style.tex <==

% \usepackage{bbm}  % for the indicator function \mathbbm{1}


% % ==== Peyman style ======================
% \usepackage[usenames, dvipsnames]{color}
% \definecolor{darkblue}{rgb}{0.0, 0.0, 0.45}

% \usepackage[colorlinks	= true,
% raiselinks	= true,
% linkcolor	= MidnightBlue, %darkblue, %
% citecolor	= Mahogany,
% urlcolor	= ForestGreen,
% pdfauthor	= {},
% pdftitle	= {},
% pdfkeywords	= {},
% pdfsubject	= {},
% plainpages	= false]{hyperref}

% \usepackage{dsfont,amssymb,subfigure, amsmath, enumitem, amsthm} %,etaremune,savesym}
% \usepackage{amsfonts,dsfont,mathtools, mathrsfs,amsthm,fancyhdr} 
% \usepackage[amssymb, thickqspace]{SIunits}
% %\usepackage{algorithm,algorithmicx}

%\usepackage{amsthm}
%%%%%%%%
\usepackage{float,graphicx}
\usepackage{amssymb,amsmath, color}
\usepackage{algorithmic, algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\usepackage{amsthm}
\usepackage{dsfont, bbm, stmaryrd}
\usepackage{hyperref}
